Spectral Heterogeneous Graph Convolutions via Positive Noncommutative Polynomials

Heterogeneous Graph Neural Networks (HGNNs) have gained significant popularity in various heterogeneous graph learning tasks. However, most existing HGNNs rely on spatial domain-based methods to aggregate information, i.e., manually selected meta-paths or some heuristic modules, lacking theoretical guarantees. Furthermore, these methods cannot learn arbitrary valid heterogeneous graph filters within the spectral domain, which have limited expressiveness. To tackle these issues, we present a positive spectral heterogeneous graph convolution via positive noncommutative polynomials. Then, using this convolution, we propose PSHGCN, a novel Positive Spectral Heterogeneous Graph Convolutional Network. PSHGCN offers a simple yet effective method for learning valid heterogeneous graph filters. Moreover, we demonstrate the rationale of PSHGCN in the graph optimization framework. We conducted an extensive experimental study to show that PSHGCN can learn diverse heterogeneous graph filters and outperform all baselines on open benchmarks. Notably, PSHGCN exhibits remarkable scalability, efficiently handling large real-world graphs comprising millions of nodes and edges. Our codes are available at https://github.com/ivam-he/PSHGCN.

==> pshgcn.tex <==
\newpage
\section{PSHGCN}
In this section, we will first define the spectral heterogeneous graph convolution, then we will propose the Positive Spectral Heterogeneous Graph
Convolutional Network (PSHGCN) via non-negative noncommutative polynomials~\cite{positive-poly}.

\subsection{Spectral Heterogeneous Graph Convolution}
Given a heterogeneous graph $G$, let $\mathbf{P}^r$ denote the shift operator of the sub-graph $G^r$. In the graph signal processing~\cite{graphsignal}, the shift operator can be given by $\{ \mathbf{A}^r\}_{r=1}^{R}$ or $\{ \mathbf{L}^r\}_{r=1}^{R}$. In other words, the shift operator $\mathbf{P}^r \in \mathbb{R}^{n \times n}$ is an adjacency matirx or a laplacian matrix of sub-graph $G^r$. Then, we can define the heterogeneous graph convolution with the notion of the shift operator.

\begin{definition}\label{h_conv}
(\textbf{Heterogeneous graph convolution}) Let $G=(V,E,\phi , \psi)$ be a heterogeneous graph with shift operator $\{\mathbf{P}^r\}_{r=1}^{R}$. Then a heterogeneous graph convolution on $G$ is a multivariate polynomial function $h(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)$.
\end{definition}

The heterogeneous graph convolution $h(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)$ is multivariate polynomial function respect to the shift operator $\{\mathbf{P}^r\}_{r=1}^{R}$. We also call it as {\bf heterogeneous graph filter} according to the notion of spectral-based GNNs~\cite{Chebnet,gcn,chebnetii}. The operation of applying the heterogeneous graph convolution to a $n$-dimensional graph signal $\mathbf{x}$ can be denoted as
\begin{equation}
    \mathbf{y}=h(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)\mathbf{x},
\end{equation}
where $\mathbf{x} \in \mathbb{R}^n$ is a graph signal and we can treat it as a column of the node features $\mathbf{X}$. We say that $\mathbf{y}$ is a filtering results of $\mathbf{x}$. In Table~\ref{tb:hgnn_with_filter}, we show some existing HGNNs with heterogeneous graph convolution.
\begin{enumerate}[leftmargin=*]
\item[$\bullet$] \textbf{GTN}~\cite{gtn} uses the Graph Transformer layer to learn the graph convolutions, which can be denoted as  $\mathbb{D}^{-1}\prod\nolimits_{k=0}^{K}\sum\nolimits_{r=0}^{R}\alpha_{r}^{(k)}\mathbf{A}^r$, where $\mathbb{D}$ denotes the multiplication of degree matrix of different convolutions for $k=1,\cdots,K-1$ and $\mathbf{A}^0$ is the identity matrix $\mathbf{I}$. GTN learns a graph convolution by learning the weights $\alpha_{r}^{(k)}$.
\item[$\bullet$] \textbf{EMRGNN}~\cite{emrgnn} utilizes the multi-relational Personalized PageRank~\cite{appnp} to learn the graph convolutions and the expression is $\sum\nolimits_{k=0}^{K}\alpha(1-\alpha)^k \left(\sum\nolimits_{r=1}^{R}\mu_r\Tilde{\mathbf{A}}^{r} \right)^k$, where $\Tilde{\mathbf{A}}$ denotes the normalized adjacency matrix with self-loops. EMRGNN approximates a graph convolution by learning the weight $\mu_r$ and setting $\alpha$ as a non-negative trade-off parameter.
\item[$\bullet$]\textbf{MHGNN}~\cite{mhgcn} simply aggregate the adjacency matrix $\mathbf{A}^r$ with learnable weights $\beta_r$ and uses $K$ GCN~\cite{gcn}-layer to achieve the graph convolution, which can denoted as $\left( 
\sum\nolimits_{r=1}^{R}\beta_r\mathbf{A}^r \right)^{K}$.
\end{enumerate}

\begin{table}[t]
\centering
\caption{Existing HGNNs with heterogeneous graph convolution.}
\begin{tabular}{@{}lll@{}}
\toprule
Method &Operator $\mathbf{P}^r$  &Filter $h$  \\ \midrule
GTN~\cite{gtn}    &$\mathbf{A}^r$  &$\mathbb{D}^{-1}\prod\nolimits_{k=0}^{K}\sum\nolimits_{r=0}^{R}\alpha_{r}^{(k)}\mathbf{A}^r$  \\
EMRGNN~\cite{emrgnn} &$\Tilde{\mathbf{A}}^r$  &$\sum\nolimits_{k=0}^{K}\alpha(1-\alpha)^k \left(\sum\nolimits_{r=1}^{R}\mu_r\Tilde{\mathbf{A}}^{r} \right)^k$ \\
MHGCN~\cite{mhgcn}  &$\mathbf{A}^r$  &$\left( 
\sum\nolimits_{r=1}^{R}\beta_r\mathbf{A}^r \right)^{K}$   \\ \bottomrule
\end{tabular}
\label{tb:hgnn_with_filter}
\end{table}

We can observe that the above methods try to approximate the heterogeneous graph convolution $h(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)$ by learning different weights. However, These methods cannot approximate arbitrary heterogeneous graph convolutions (i.e., the multivariate polynomial function $h$) and have no discussion or constraints on the output of the convolution $h$.

\subsection{Positive Spectral Heterogeneous Graph Convolution Network}
We use the most general multivariate polynomial $g$ ~\cite{multi_poly} with monomial basis to approximate arbitrary heterogeneous graph convolutions $h$.
\begin{equation}\label{eq:g}
g(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)=w_0\mathbf{I}+\sum\limits_{k=1}^{K}\sum\limits_{r_1,\cdots,r_K\in R}w_{r_1,\cdots,r_k}\mathbf{P}^{r_1}\cdots\mathbf{P}^{r_k},
\end{equation}
where $w$ denotes the polynomial coefficients and $k$ is the order of the polynomial. For example, a $2$-order polynomial $g$ with two variables can be denoted as $g(\mathbf{P}^1,\mathbf{P}^2)=w_0\mathbf{I}+w_1\mathbf{P}^{1}+w_2\mathbf{P}^{2}+w_3 \mathbf{P}^{1}\mathbf{P}^{1}+w_4 \mathbf{P}^{1} \mathbf{P}^{2}+w_5 \mathbf{P}^{2} \mathbf{P}^{1}+w_6\mathbf{P}^{2}\mathbf{P}^{2}$. According to the polynomial approximation theory, the multivariate polynomial $g$ can approximate arbitrary heterogeneous graph convolution $h$ when $K \rightarrow \infty$.  In theory, the number of the coefficients $w$ is $1+R+R^2+\cdots+R^K=\frac{R^{K+1}-1}{R-1}$ increasing exponentially. However, in practice, many $\mathbf{P}^i\mathbf{P}^j=\mathbf{0}$ allowing us to eliminate them, so the number of the coefficients does not increase exponentially with $K$. Notably, the multivariate polynomial $g$ is a noncommutative polynomial~\cite{positive-poly} since the two shift operator $\mathbf{P}^i$ and $\mathbf{P}^j$ are not commutative (i.e., $\mathbf{P}^i\mathbf{P}^j \neq \mathbf{P}^j\mathbf{P}^i$).


\begin{figure*}[t]
    \centering
    \includegraphics[height=6.2cm]{fig/pshgcn.pdf}
    %\vspace{0mm}
    \caption{An illustration of the proposed PSHGCN.}
    \label{fig:scheme}
\end{figure*}

Similar to the filtering operation of homogeneous spectral-based GNNs (Equation~\eqref{spec_gnn}), the operation $\mathbf{y}=h(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)\mathbf{x}$ in heterogeneous graphs should also satisfy some constraints. We denote $h(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)$ as $\mathbf{H}\in \mathbb{R}^{n\times n}$. Following the spectral-based GNN BernNet~\cite{bernnet}, a simple and intuitive constraint is that $\mathbf{H}$ should be a positive semidefinite matrix.  We emphasize that this constraint is consistent since the filtering operation can be denoted as $\mathbf{y}=\mathbf{Q}\mathbf{\Sigma}\mathbf{Q}^{\top}\mathbf{x}$, where $\mathbf{Q}\mathbf{\Sigma}\mathbf{Q}^{\top}=\mathbf{H}$ is the eigendecomposition of $\mathbf{H}$ and $\mathbf{Q}^{\top}\mathbf{x}$ can be interpreted as the graph fourier transform on heterogeneous graphs. In order to ensure that $\mathbf{H}$ is positive semidefinite, we must use the form of sum of squares. 
\begin{equation}
    h(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)=\sum\limits_{i}g_i(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)^{\top}g_i(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R),
\end{equation}
Specifically, we have the following Theorem:

\begin{theorem}\label{th_sos_posi}
~\cite{positive-poly} Suppose $h$ is a noncommutative symmetric polynomial. If $h$ is a sum of squares, then $h$ is matrix-positive. If $h$ is matrix-positive
a sum of squares.
\end{theorem}
The "matrix-positive" means the resulting matrix $\mathbf{H}$ is positive semidefinite. Theorem~\ref{th_sos_posi} guarantees that the output of the heterogeneous graph filter $h$ is positive semidefinite, and we also call it a valid filter. Using the valid filter, we propose the Positive Spectral Heterogenegous Graph Convolution Network (PSHGCN) and the filtering operation of PSHGCN can be denoted as
\begin{equation}
    \mathbf{y}=\sum\limits_{i}g_i(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)^{\top}g_i(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)\mathbf{x}.
\end{equation}
In general, $g_i$ is a multivariate polynomial defined in Equation~\eqref{eq:g}. We simplify the number of $g_i$ by using only one multivariate polynomial $g$ to approximate the graph convolution $h$. As illustrated in Figure~\ref{fig:scheme}, our PSHGCN approximated an arbitrary positive semidefinite heterogeneous graph convolution $\mathbf{H}$ by the sum of squares $g(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)^{\top} g(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)$. The structure of PSHGCN can be denoted as
\begin{equation}
    \mathbf{Z}=f^{\prime}_{\theta}(\mathbf{Y}), \mathbf{Y}=g(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)^{\top} g(\mathbf{P}^1,\mathbf{P}^2,\cdots,\mathbf{P}^R)f_{\theta}(\mathbf{X}), 
\end{equation}
where $g$ is a multivariate polynomial defined in Equation~\eqref{eq:g}, $f_{\theta}(\cdot)$ and $f^{\prime}_{\theta}(\cdot)$ denote Multi-layer Perceptron (MLP) used for feature extraction and downstream learning task, repectively.







